Towards Poisoning Fair Representations

Fair machine learning seeks to mitigate model prediction bias against certain demographic subgroups such as elder and female. Recently, fair representation learning (FRL) trained by deep neural networks has demonstrated superior performance, whereby representations containing no demographic information are inferred from the data and then used as the input to classification or other downstream tasks. Despite the development of FRL methods, their vulnerability under data poisoning attack, a popular protocol to benchmark model robustness under adversarial scenarios, is under-explored. Data poisoning attacks have been developed for classical fair machine learning methods which incorporate fairness constraints into shallow-model classifiers. Nonetheless, these attacks fall short in FRL due to notably different fairness goals and model architectures. This work proposes the first data poisoning framework attacking FRL. We induce the model to output unfair representations that contain as much demographic information as possible by injecting carefully crafted poisoning samples into the training data. This attack entails a prohibitive bilevel optimization, wherefore an effective approximated solution is proposed. A theoretical analysis on the needed number of poisoning samples is derived and sheds light on defending against the attack. Experiments on benchmark fairness datasets and state-of-the-art fair representation learning models demonstrate the superiority of our attack.

==> subfiles/1_intro_old.tex <==
\section{Introduction}





\pan{[1]. Scalable Infomin Learning, NeurIPS 2022}
\pan{Why is FLD approximation good enough?}
\pan{Why previous data positioning method cannot be used here?}
\pan{T-SNE visualization?}

% Fair machine learning is important

Machine learning algorithms have found a proliferation of applications in automated decision-making in high-stakes domains 
such as applicant screening in job markets and credit risk analysis.
However, it was observed that many machine learning algorithms tend to discriminate certain demographic subgroups such as {females} when making decisions due to commonly existing bias in training data  \cite{barocas2016big, buolamwini2018gender, dressel2018accu}.  
For instance, when most records of {physicians} are {male} in a dataset, 
an applicant screening algorithm trained with this data may determine someone's eligibility for a {physician} position based on their gender instead of education background or professional experience, which leads to \textit{unfair} outcomes for female applicants.
Conceptually, 
the phenomenon that machine learning algorithms make biased decisions across different demographic subgroups and give favorable predictions for some particular subgroups is termed as \textit{algorithmic (un)fairness}, memberships of demographic subgroups are often considered as \textit{sensitive information} and denoted by \textit{sensitive features}, and research on achieving algorithmic fairness is known as \textit{fair machine learning}. 




The rapid growing area of fair machine learning has accumulated a vast literature that proposes various fairness notions and attempts to achieve them~\cite{pedreshi2008discrimination, dwork2011fairness, hardt2016equality, chouldechova2020snapshot}. 
Fairness notions are requirements that a model should satisfy
and are usually fulfilled by imposing corresponding penalties or constraints \citep{donini2018empirical}. 
Fairness on \textit{shallow} models such as logistic regression \citep{kamishima2011fairness} and support vector machine \citep{zafar2017fairness} has been well-studied, which we refer to as \textit{classical fair machine learning}. 
Recently, \textit{fair representation learning} relying on deep neural networks \cite{xie2017controllable, madras2018learning, moyer2018invariant, creager2019flexibly, sarhan2020fairness, wang2021fair} has attracted great attention. These works learn representations that contain minimal information of sensitive features. When data representations from different demographic subgroups are similar to each other, any classifiers acting on these representations will be \textit{agnostic} to the membership of demographic subgroups, achieving fairness in a variety of settings thereof. 
Compared to classical fair machine learning, fair representation learning often achieves better transferability on downstream tasks \cite{creager2019flexibly}. 
% \pan{This paragraph can be shortened.}

% All these methods together have greatly advanced the progress of mitigating discriminatory decisions made by machine learning algorithms.  


% Specifically, fair representations are usually learned by achieving
% some types of objectives that satisfy certain fairness constraints. 

Despite the success of fair machine learning methods, not much is known about their vulnerability under data poisoning attacks until very recent studies \cite{chang2020adversarial, solans2021poisoning, mehrabi2021exacerbating}. 
Data poisoning attacks aim to maliciously control a model's behavior to achieve some goals by injecting poisoned training samples to influence its training and are widely used to benchmark the vulnerability and robustness of machine learning models \cite{huang2020metapoison, geiping2020witches, koh2022stronger}. 
Recently researchers successfully attacked classical fair machine learning methods such as fair logistic regression \citep{solans2021poisoning, mehrabi2021exacerbating}
and degraded their fairness performance. 
But 
it is still an open question whether fair representation learning suffers from a similar threat. 

% However, whether fair representation learning suffers from a similar threat or not has not be studied yet.
% Meanwhile, it is found that an attack aiming to reduce accuracy does not harm fairness metrics in general, 
% highlighting the importance of studies on understanding the vulnerability of fair machine learning. \citet{mehrabi2021exacerbating} further revealed that when attacking a logistic regression,  traditional poisoning attacks to reduce accuracy do not perform well on degrading the fairness, 
% underpinning the necessity of designing specialized poisoning attacks for different fair machine learning tasks \citep{chhabra2021fairness, chhabra2022robust}. 


Notwithstanding, existing attacks on classical fair machine learning cannot be readily applied to fair representation learning. 
These attacks are either optimization-based or heuristic-based. Optimization-based attacks require the victim model being attacked to be simple enough (e.g., convex) \citep{solans2021poisoning, mehrabi2021exacerbating}; heuristics, on the other hand, have no guarantees of their success \pan{ours is also heuristics? is this a strong enough argu?}. 
% rely on the convexity of victim models that are attacked or require intensive computations of second-order derivatives. 
For fair representation learning that involves deep neural networks, optimization-based attacks are neither applicable nor affordable due to the non-convex nature \citep{huang2020metapoison, geiping2020witches}, while heuristic attacks are often less effective in practice \citep{mehrabi2021exacerbating}. 
% \tianci{
% Another challenge lies in the attack goal.
% Unlike classical fair machine learning, fair representation learning does not require specific labels (decisions to make) during training \cite{creager2019flexibly}.
% This makes it unsuitable to directly adopt label-specific attack goals from existing works on poisoning classical fair machine learning.
% } \pan{I do not understand this. I think we are still working on supervised learning tasks?}




% \begin{figure}[tb]
% \centering
% \includegraphics[width=0.8\linewidth]{figures/flow4.pdf}
% \caption{
% Framework of data poisoning attack (shown in red) on fair representation learning. Note that some
% irrelevant components such as class labels are not included.
% The attacker poisons training data to contaminate the victim training (solid lines), aiming to learn unfair representation $\zv$ for target data  (dotted lines) such that its mutual information (MI) to sensitive feature $a$ is maximized. The MI is supposed to be close to zero on fair representations before the attack.  
% }
% \label{fig:flow}
% \end{figure}



\begin{wrapfigure}{R}{8.5cm}
\centering
\includegraphics[width=\linewidth]{figures/workflow.pdf}
\caption{
% \small
Framework of data poisoning attack (shown in red) on fair representation learning. Note that some
irrelevant components such as class labels are not included.
The attacker poisons training data to contaminate the victim training (solid lines), aiming to learn unfair representation $\zv$ for target data  (dotted lines) such that its mutual information (MI) to sensitive feature $a$ is maximized. The MI is supposed to be close to zero on fair representations before the attack.  
}
 \label{fig:flow} \vspace{-0.1in}
\end{wrapfigure}


In this paper,
we propose the first data poisoning attack on fair representation learning as outlined in Figure \ref{fig:flow}.  
{As the first work on this topic, we focus on binary sensitive features
given their importance in fair representation learning \cite{madras2018learning, moyer2018invariant, zhao2019conditional}.
}
Ideal fair representations should contain no sensitive information, i.e., 
their mutual information (MI) with the sensitive feature should be zero. 
Henceforth, we seek to learn \textit{unfair} representations for target data that has MI with the sensitive feature as large as possible. 
This goal entails a prohibitive bilevel optimization, where challenges lie in two-fold.  
Firstly, MI lacks an analytic form, making its maximization challenging. 
{
It is known that in binary classification, the 
negative binary-cross-entropy (BCE) loss of any classifier is a lower bound for MI between the label and the features \cite{poole2019variational}. Based on this fact, we propose to reduce the MI maximization problem to the problem of minimizing the BCE loss of a classifier that predicts sensitive feature from the representations.
By connecting the minimal BCE loss the classifier can achieve with the data separability, we further reduce the problem to the task of maximizing the separability of different classes of data, which has a closed form solution. 
}
% It is known that for any classifier to predict 
% {
% Recalling that the negative binary-cross-entropy (BCE) loss of a classifier to predict the sensitive feature from learned representation is a lower bound for the MI \cite{poole2019variational}, we reduce the MI maximization problem to minimizing the optimal BCE loss of the classifier, which is further replaced by maximizing separability of different classes of data. 
% }
Secondly, the representation is learned by some deep neural network and its dependency on poisoning samples is impossible to track exactly. As a result, one cannot identify what poisoning samples will induce the victim to produce unfair representations on target data even knowing how they should look like. 
{We build an effective approximated solution upon existing tools with better stealthiness of our attack consideration.}
{
To our best knowledge, we are not only the first to poison fair representation learning, but also the first to introduce MI explicitly \pan{Here we should be careful. Is there any work that uses classification as the goal? Also, in the intro, we did not mention anything related to FLD.} as an attack goal towards fair machine learning. This is one of the most significant contributions of our work.
}
Section \ref{sec:method} discusses these in details.

% \begin{table}[tb]
% \begin{center}
% \caption{
% % Will be shown s
% Three levels of optimization (in different colors) in poisoning fair representation learning. \pan{It is better to have a figure or equation? not intuitive enough}
% % Detailed formulations are given in Section \ref{sec:method}.
% }\label{tab:goal}

% \resizebox{0.9\linewidth}{!}{
% % \renewcommand{\tabcolsep}{6pt}
% \begin{tabular}{
% p{0.33\linewidth}  
% p{0.33\linewidth}  
% p{0.33\linewidth}
% }
% \toprule
% \textbf{\textcolor{blue}{Upper-level} Objective} & 
% \textbf{\textcolor{orange}{Middle-level} Objective} & 
% \textbf{\textcolor{purple}{Lower-level } Objective} \\
% \midrule
% \textit{Identify the optimal \textcolor{blue}{poisoning samples} to 
% make the \textcolor{orange}{classification} easier. }
% & 
% \textit{Identify the optimal \textcolor{orange}{classifier} to predict sensitive features from 
% \textcolor{purple}{the learned representations}. }
% & 
% \textit{Identify the optimal \textcolor{purple}{representation} learner on \textcolor{blue}{poisoned training data}.}
% \\
% \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table}


Practical data poisoning attacks should rely on only a few poisoning samples, as using more poisoning samples will increase the chance of an attack being detected \cite{geiping2020witches, huang2020metapoison, koh2022stronger}. 
In Section \ref{sec:theorems} we derive a theoretical minimal number of poisoning samples required by the attack to succeed under regular conditions. This bound applies to GradMatch \cite{geiping2020witches} \pan{did we say anything related to GradMatch in the pipeline?}, a state-of-the-art general-purpose data poisoning attack and may be of independent interest to all of its users. 
{This theoretical analysis is another main contribution of our work.}
Results obtained from extensive experiments (as shown in Section \ref{sec:experiment}) demonstrate that the proposed method delivers strong attacks on 
four representative fair representation learning methods, with the use of as few as 5\% of training data as poisoning samples. 
In the remaining part of this paper, we review the literature in Section \ref{sec:background}, and discuss the future work in Section \ref{sec:conclusion}. 



% \begin{wrapfigure}{R}{9.5cm}
% \centering
% \includegraphics[width=0.6\linewidth]{figures/flow.pdf}
% \caption{\small Overview of fair representation attack.}
%  \label{fig:flow} \vspace{-0.1in}
% \end{wrapfigure}



% \pan{Maybe, we can clarify more the key insights and techniques used for simplifying opt and analysis in the intro. Any ways to explain why the problem is by nature 3-level opt? why it can be simplied and approxiated? the significance of the analysis?}





% As the first work on poisoning fair representation learning algorithms, 
% the contribution of this work is in {three}-fold.
% % First, we propose the first formulation of poisoning attack on fair representation learning aiming at maximizing the predictiveness of sensitive features from the fair representation. 
% First, we formulate the task of poisoning attack on fair representation  learning as a tri-level optimization problem. The goal is to find the optimal data perturbation so as to maximize the predictiveness of sensitive features from the fair representations using some simple classifiers.
% % Second, we provide an effective way to achieve the attack goal approximately.  
% Second, given the non-convexity of victim and the lack of analytic measure for predictiveness, the original tri-level optimization problem is intractable, and we propose an effective way to relax the problem into a solvable format.
% % Third, we provide an adaptive way to regulate the attacker when crafting poisoning samples by the use of a statistical tool in high dimensional feature selection, which forcing the attacker to make only useful perturbations. 
% Third, we provide a theoretical lower bound on the number of poisoning samples needed to guarantee the predictiveness towards sensitive features under regular conditions.
% % , which establishes a rigorous foundation for our method. 
% In evaluation, we design several ways to attack victims trained with different-sized data. As the first work on fair representation learning attack, there are no baselines that follow the same problem setting. Nonetheless, we compare the proposed methods with state-of-the-art poisoning attacks on classical fair machine learning and demonstrate the superiority of the proposed methods. 
% %Extensive experiments show that the proposed methods outperform a recent heuristic poisoning attack on classical fair machine learning by a large margin. 
% By checking how the proposed methods perturb data when attacking a victim model, we provide insights into the robustness of existing fair representation learning methods.


% The paper proceeds as follows. In Section \ref{sec:background}, we provide background knowledge in fair machine learning, fair representation learning, and data poisoning attacks. In Section \ref{sec:method}, we formally propose the framework of poisoning fair representation learning and give theoretical analysis. 
% In Section \ref{sec:experiment}, we illustrate our algorithm and show its outstanding performance compared to 
% a recent heuristic poisoning attack method on traditional fair machine learning. 
% Section \ref{sec:conclusion} concludes the paper. 
% We defer the proofs, some technical details, and supplementary results to the appendix.






% Unfortunately, techniques applied in 
% rely on are usually computational demanding \tianci{citation} or are solely heuristic without theoretical foundation \tianci{more references}, which are not suitable for attacking . These two limitations restrict their effectiveness in attacking fair representation. Fair representation learning use deep neural networks as backbones \citep{moyer2018invariant, zhao2019conditional}, which are known more challenging and require new attacking methods due to their non-convexity \citep{huang2020metapoison, geiping2020witches}. 
% Motivated by the lack of existing work on 






% Meanwhile, the success and ubiquity of representation learning in machine learning inspire 
% otivated by 





% \hengtong{
% If we are the first to study the poisoning attack on fair representation, then we may add extra discussion on
% \begin{itemize}
% \item 
% Why existing fairness attack methods cannot work? \tianci{check existing works to find 2 baseline heuristics. }
% \item
% Highlight that we are the first one and the challenge
% \end{itemize}
% }


